Towards a Unified Framework for Adaptable Problematic Content Detection via Continual Learning

Detecting problematic content, such as hate speech, is a multifaceted and ever-changing task, influenced by social dynamics, user populations, diversity of sources, and evolving language. There has been significant efforts, both in academia and in industry, to develop annotated resources that capture various aspects of problematic content. Due to researchers' diverse objectives, the annotations are inconsistent and hence, reports of progress on detection of problematic content are fragmented. This pattern is expected to persist unless we consolidate resources considering the dynamic nature of the problem. We propose integrating the available resources, and leveraging their dynamic nature to break this pattern. In this paper, we introduce a continual learning benchmark and framework for problematic content detection comprising over 84 related tasks encompassing 15 annotation schemas from 8 sources. Our benchmark creates a novel measure of progress: prioritizing the adaptability of classifiers to evolving tasks over excelling in specific tasks. To ensure the continuous relevance of our framework, we designed it so that new tasks can easily be integrated into the benchmark. Our baseline results demonstrate the potential of continual learning in capturing the evolving content and adapting to novel manifestations of problematic content.

==> old_sections/old_abstract.tex <==
\subsection{V1}
Detecting problematic content is a multifaceted and ever-changing task, influenced by social dynamics, creative users, diversity of sources, and evolving language. World events, such as wars or pandemics, create new content and content types, and countries, platforms and populations continually move the boundaries of problematic content. The diversity in annotation guidelines and the extensive range of resources created by the community reflect the inherent variability in dealing with problematic content. Continual learning is a promising framework to handle the evolving content in problematic text detection. It enables models to continuously accumulate knowledge and adapt to emerging content types, addressing challenges posed by dynamic content creators, new events, and varying perspectives on problematic content. In this paper, we propose approaching the detection of problematic content as a continual learning problem, taking advantage of its dynamic and adaptable characteristics. We define the essential characteristics of an ideal model for detecting problematic content and create a continual learning benchmark comprising over 100+ related tasks and evaluation metrics that represent these criteria. These tasks encompass 15 annotation schemas, capturing diverse aspects of problematic content from eight different platforms. Through our experiments, we explore continual learning methods and their effectiveness in addressing the challenges of problematic content detection. Our research provides valuable insights for developing more adaptable and scalable systems.


\subsection{V2}

Detecting problematic content is a multifaceted and ever-changing task, influenced by social dynamics, user populations, diversity of sources, and evolving language. The community of researchers has been making significant efforts to develop annotated resources that capture various aspects of problematic content. Due to their diverse objectives, the annotations are inconsistent and hence, reports of progress on automatic detection of problematic content  are fragmented. This pattern is expected to persist unless we integrate resources considering their dynamic nature. 
In this paper, we introduce a continual learning benchmark and framework for problematic content detection comprising over 100 related tasks encompassing 15 annotation schemas from eight sources. To ensure the continuous relevance of our framework, we have designed it so that new tasks can easily be integrated into the benchmark. Through our experiments, we demonstrate the promise of continual learning capturing the evolving content in problematic text detection and its advantage over static approaches when it comes to the detection of novel content types. 

\subsection{V3}
Detecting problematic content is a multifaceted and ever-changing task, influenced by social dynamics, user populations, diversity of sources, and evolving language. The community of researchers has been making significant efforts to develop annotated resources that capture various aspects of problematic content. Due to their diverse objectives, the annotations are inconsistent and hence, reports of progress on automatic detection of problematic content  are fragmented. This pattern is expected to persist unless we integrate resources considering their dynamic nature. 
We propose integrating the published resources, and leveraging their dynamic nature to break this pattern. In this paper, we introduce a continual learning benchmark and framework for problematic content detection comprising over 100 related tasks encompassing 15 annotation schemas from eight sources. To ensure the continuous relevance of our framework, we have designed it so that new tasks can easily be integrated into the benchmark. Through our experiments, we demonstrate the promise of continual learning capturing the evolving content in problematic text detection and its advantage over static approaches when it comes to the detection of novel content types. 

==> tables/dataset_overview.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccc}
\multicolumn{1}{c|}{Dataset}             & \multicolumn{1}{c|}{Tasks}                                                                                                             & Questions                                                                                                                                                                                                                                 \\ \hline
\multicolumn{1}{c|}{Personal attack(PA)} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}PA, Quoted PA, \\ Targeted at recipient PA,\\  Targeted at third party TA\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Does this comment contain a {[}personal attack/\\  personal attack that is being quoted/\\  a personal attack targeted at recipient of the message/ \\ personal attack targeted at a third-party{]}?\end{tabular} \\ \hline
\multicolumn{1}{l}{}                     & \multicolumn{1}{l}{}                                                                                                                   & \multicolumn{1}{l}{}                                                                                                                                                                                                                     
\end{tabular}
\caption{}
\label{tab:dataset-overview}
\end{table}

==> tables/instant-two-part.tex <==
\begin{tabular}{rlll}
\toprule
auc & dataset & task & model \
\midrule
0.975141 & abusive & abusive & BART-Adapter-Vanilla \
0.972513 & abusive & abusive & BART-BiHNet+Reg \
\hline
0.858683 & abusive & hateful & BART-Adapter-Vanilla \
0.864749 & abusive & hateful & BART-BiHNet+Reg \
\hline
0.887943 & cad & affiliationdirectedabuse & BART-Adapter-Vanilla \
0.879390 & cad & affiliationdirectedabuse & BART-BiHNet+Reg \
\hline
0.780956 & cad & identitydirectedabuse & BART-Adapter-Vanilla \
0.799686 & cad & identitydirectedabuse & BART-BiHNet+Reg \
\hline
0.878956 & cad & persondirectedabuse & BART-Adapter-Vanilla \
0.880668 & cad & persondirectedabuse & BART-BiHNet+Reg \
\hline
0.828820 & dygen & hate & BART-Adapter-Vanilla \
0.762699 & dygen & hate & BART-BiHNet+Reg \
\hline
0.870509 & ghc & hd & BART-Adapter-Vanilla \
0.872039 & ghc & hd & BART-BiHNet+Reg \
\hline
0.893579 & ghc & vo & BART-Adapter-Vanilla \
0.899036 & ghc & vo & BART-BiHNet+Reg \
\hline
0.940574 & hate & hateful & BART-Adapter-Vanilla \
0.940949 & hate & hateful & BART-BiHNet+Reg \
\hline
0.979880 & jigsaw & identity-attack & BART-Adapter-Vanilla \
0.982487 & jigsaw & identity-attack & BART-BiHNet+Reg \
\hline
0.951626 & jigsaw & insult & BART-Adapter-Vanilla \
0.949777 & jigsaw & insult & BART-BiHNet+Reg \
\hline
0.977025 & jigsaw & obscene & BART-Adapter-Vanilla \
0.978208 & jigsaw & obscene & BART-BiHNet+Reg \
\hline
0.987871 & jigsaw & threat & BART-Adapter-Vanilla \
0.989349 & jigsaw & threat & BART-BiHNet+Reg \
\hline
0.938429 & jigsaw & toxicity & BART-Adapter-Vanilla \
0.930403 & jigsaw & toxicity & BART-BiHNet+Reg \
\hline
0.962485 & personal-attack & a & BART-Adapter-Vanilla \
0.961693 & personal-attack & a & BART-BiHNet+Reg \
\hline
0.972592 & personal-attack & ra & BART-Adapter-Vanilla \
0.972671 & personal-attack & ra & BART-BiHNet+Reg \
\hline
\end{tabular}

\begin{tabular}{rlll}
\toprule
auc & dataset & task & model \
\midrule
0.949232 & personal-attack & tpa & BART-Adapter-Vanilla \
0.934629 & personal-attack & tpa & BART-BiHNet+Reg \
\hline
0.824417 & ucc & antagonize & BART-Adapter-Vanilla \
0.830485 & ucc & antagonize & BART-BiHNet+Reg \
\hline
0.785604 & ucc & condescending & BART-Adapter-Vanilla \
0.776889 & ucc & condescending & BART-BiHNet+Reg \
\hline
0.825034 & ucc & dismissive & BART-Adapter-Vanilla \
0.819899 & ucc & dismissive & BART-BiHNet+Reg \
\hline
0.848341 & ucc & generalisation & BART-Adapter-Vanilla \
0.875159 & ucc & generalisation & BART-BiHNet+Reg \
\hline
0.860923 & ucc & generalisation-unfair & BART-Adapter-Vanilla \
0.860750 & ucc & generalisation-unfair & BART-BiHNet+Reg \
\hline
0.723211 & ucc & healthy & BART-Adapter-Vanilla \
0.720583 & ucc & healthy & BART-BiHNet+Reg \
\hline
0.837135 & ucc & hostile & BART-Adapter-Vanilla \
0.855591 & ucc & hostile & BART-BiHNet+Reg \
\hline
0.715202 & ucc & sarcastic & BART-Adapter-Vanilla \
0.710375 & ucc & sarcastic & BART-BiHNet+Reg \
\hline
\bottomrule
\end{tabular}

==> tables/old/fs_buggy.tex <==
\begin{tabular}{llll}
\toprule
task--name & task--detail & nf1 & alg \\
\midrule
BAD2 & singlelabel & 0.627 & CL \\
BAD2 & singlelabel & 0.713 & MTL \\
BAD2 & singlelabel & 0.629 & Vanilla \\ 
 \hline
BAD4 & singlelabel & 0.537 & CL \\
BAD4 & singlelabel & 0.715 & MTL \\
BAD4 & singlelabel & 0.572 & Vanilla \\ 
 \hline
cmsb & sexist & 0.792 & CL \\
cmsb & sexist & 0.859 & MTL \\
cmsb & sexist & 0.866 & Vanilla \\ 
 \hline
conan & disabled & 0.964 & CL \\
conan & disabled & 0.918 & MTL \\
conan & disabled & 0.960 & Vanilla \\ 
 \hline
conan & jews & 0.972 & CL \\
conan & jews & 0.928 & MTL \\
conan & jews & 0.986 & Vanilla \\ 
 \hline
conan & lgbt & 0.888 & CL \\
conan & lgbt & 0.788 & MTL \\
conan & lgbt & 0.906 & Vanilla \\ 
 \hline
conan & migrant & 0.870 & CL \\
conan & migrant & 0.850 & MTL \\
conan & migrant & 0.914 & Vanilla \\ 
 \hline
conan & muslims & 0.806 & CL \\
conan & muslims & 0.870 & MTL \\
conan & muslims & 0.934 & Vanilla \\ 
 \hline
conan & poc & 0.626 & CL \\
conan & poc & 0.856 & MTL \\
conan & poc & 0.930 & Vanilla \\ 
 \hline
conan & woman & 0.920 & CL \\
conan & woman & 0.938 & MTL \\
conan & woman & 0.948 & Vanilla \\ 
 \hline
dygen & african & 0.853 & CL \\
dygen & african & 0.760 & MTL \\
dygen & african & 0.978 & Vanilla \\ 
 \hline
dygen & animosity & 0.536 & CL \\
dygen & animosity & 0.787 & MTL \\
dygen & animosity & 0.901 & Vanilla \\ 
 \hline
dygen & arab & 0.893 & CL \\
dygen & arab & 0.784 & MTL \\
dygen & arab & 0.972 & Vanilla \\ 
 \hline
dygen & asi & 0.851 & CL \\
dygen & asi & 0.826 & MTL \\
dygen & asi & 0.979 & Vanilla \\ 
 \hline
dygen & asylum & 0.757 & CL \\
dygen & asylum & 0.851 & MTL \\
dygen & asylum & 0.979 & Vanilla \\ 
 \hline
dygen & bis & 0.487 & CL \\
dygen & bis & 0.857 & MTL \\
dygen & bis & 0.980 & Vanilla \\ 
 \hline
dygen & bla & 0.573 & CL \\
dygen & bla & 0.764 & MTL \\
dygen & bla & 0.905 & Vanilla \\ 
 \hline
dygen & dehumanization & 0.556 & CL \\
dygen & dehumanization & 0.862 & MTL \\
dygen & dehumanization & 0.947 & Vanilla \\ 
 \hline
dygen & derogation & 0.611 & CL \\
dygen & derogation & 0.666 & MTL \\
dygen & derogation & 0.654 & Vanilla \\ 
 \hline
dygen & dis & 0.781 & CL \\
dygen & dis & 0.875 & MTL \\
dygen & dis & 0.955 & Vanilla \\ 
 \hline
dygen & for & 0.595 & CL \\
dygen & for & 0.783 & MTL \\
dygen & for & 0.971 & Vanilla \\ 
 \hline
dygen & gay & 0.702 & CL \\
dygen & gay & 0.812 & MTL \\
dygen & gay & 0.966 & Vanilla \\ 
 \hline
dygen & gendermin & 0.524 & CL \\
dygen & gendermin & 0.827 & MTL \\
dygen & gendermin & 0.976 & Vanilla \\ 
 \hline
dygen & hispanic & 0.746 & CL \\
dygen & hispanic & 0.897 & MTL \\
dygen & hispanic & 0.983 & Vanilla \\ 
 \hline
dygen & hitler & 0.907 & CL \\
dygen & hitler & 0.907 & MTL \\
dygen & hitler & 0.982 & Vanilla \\ 
 \hline
dygen & immig & 0.700 & CL \\
dygen & immig & 0.837 & MTL \\
dygen & immig & 0.964 & Vanilla \\ 
 \hline
dygen & indig & 0.875 & CL \\
dygen & indig & 0.889 & MTL \\
dygen & indig & 0.978 & Vanilla \\ 
 \hline
dygen & jew & 0.622 & CL \\
dygen & jew & 0.813 & MTL \\
dygen & jew & 0.950 & Vanilla \\ 
 \hline
dygen & lgbtq & 0.739 & CL \\
dygen & lgbtq & 0.882 & MTL \\
dygen & lgbtq & 0.992 & Vanilla \\ 
 \hline
dygen & mus & 0.633 & CL \\
dygen & mus & 0.784 & MTL \\
dygen & mus & 0.958 & Vanilla \\ 
 \hline
dygen & nazis & 0.867 & CL \\
dygen & nazis & 0.941 & MTL \\
dygen & nazis & 0.991 & Vanilla \\ 
 \hline
dygen & pol & 0.717 & CL \\
dygen & pol & 0.849 & MTL \\
dygen & pol & 0.978 & Vanilla \\ 
 \hline
dygen & ref & 0.851 & CL \\
dygen & ref & 0.898 & MTL \\
dygen & ref & 0.969 & Vanilla \\ 
 \hline
dygen & russian & 0.694 & CL \\
dygen & russian & 0.806 & MTL \\
dygen & russian & 0.983 & Vanilla \\ 
 \hline
dygen & support & 0.671 & CL \\
dygen & support & 0.794 & MTL \\
dygen & support & 0.958 & Vanilla \\ 
 \hline
dygen & threatening & 0.728 & CL \\
dygen & threatening & 0.849 & MTL \\
dygen & threatening & 0.963 & Vanilla \\ 
 \hline
dygen & trans & 0.594 & CL \\
dygen & trans & 0.662 & MTL \\
dygen & trans & 0.947 & Vanilla \\ 
 \hline
dygen & trav & 0.732 & CL \\
dygen & trav & 0.816 & MTL \\
dygen & trav & 0.979 & Vanilla \\ 
 \hline
dygen & wom & 0.739 & CL \\
dygen & wom & 0.787 & MTL \\
dygen & wom & 0.917 & Vanilla \\ 
 \hline
hatecheck & black & 0.708 & CL \\
hatecheck & black & 0.845 & MTL \\
hatecheck & black & 0.928 & Vanilla \\ 
 \hline
hatecheck & disabled & 0.909 & CL \\
hatecheck & disabled & 0.920 & MTL \\
hatecheck & disabled & 0.965 & Vanilla \\ 
 \hline
hatecheck & gay & 0.826 & CL \\
hatecheck & gay & 0.882 & MTL \\
hatecheck & gay & 0.920 & Vanilla \\ 
 \hline
hatecheck & hate & 0.866 & CL \\
hatecheck & hate & 0.780 & MTL \\
hatecheck & hate & 0.627 & Vanilla \\ 
 \hline
hatecheck & immigrants & 0.756 & CL \\
hatecheck & immigrants & 0.898 & MTL \\
hatecheck & immigrants & 0.936 & Vanilla \\ 
 \hline
hatecheck & muslims & 0.660 & CL \\
hatecheck & muslims & 0.882 & MTL \\
hatecheck & muslims & 0.973 & Vanilla \\ 
 \hline
hatecheck & trans & 0.791 & CL \\
hatecheck & trans & 0.962 & MTL \\
hatecheck & trans & 0.941 & Vanilla \\ 
 \hline
hatecheck & women & 0.700 & CL \\
hatecheck & women & 0.944 & MTL \\
hatecheck & women & 0.893 & Vanilla \\ 
 \hline
misogyny & singlelabel & 0.811 & CL \\
misogyny & singlelabel & 0.906 & MTL \\
misogyny & singlelabel & 0.904 & Vanilla \\ 
 \hline
single & singlelabel & 0.963 & CL \\
single & singlelabel & 0.894 & MTL \\
single & singlelabel & 0.936 & Vanilla \\ 
 \hline
single--adversarial & singlelabel & 0.902 & CL \\
single--adversarial & singlelabel & 0.873 & MTL \\
single--adversarial & singlelabel & 0.730 & Vanilla \\ 
 \hline
stormfront & singlelabel & 0.786 & CL \\
stormfront & singlelabel & 0.762 & MTL \\
stormfront & singlelabel & 0.747 & Vanilla \\ 
 \hline
us--election & biden & 0.480 & CL \\
us--election & biden & 0.442 & MTL \\
us--election & biden & 0.391 & Vanilla \\ 
 \hline
us--election & hof & 0.773 & CL \\
us--election & hof & 0.837 & MTL \\
us--election & hof & 0.707 & Vanilla \\ 
 \hline
us--election & trump & 0.416 & CL \\
us--election & trump & 0.271 & MTL \\
us--election & trump & 0.381 & Vanilla \\ 
 \hline
\bottomrule
\end{tabular}

==> tables/old/proof_concept_few.tex <==
\begin{tabular}{llll}
\toprule
task--name & task--detail & nf1 & alg \\
\midrule
cmsb & sexist & 0.872 & CL \\
cmsb & sexist & 0.877 & MTL \\
cmsb & sexist & 0.876 & Vanilla \\
cmsb & sexist & 0.878 & pretrained \\ 
 \hline
ucc & antagonize & 0.954 & CL \\
ucc & antagonize & 0.952 & MTL \\
ucc & antagonize & 0.951 & Vanilla \\
ucc & antagonize & 0.952 & pretrained \\ 
 \hline
ucc & condescending & 0.940 & CL \\
ucc & condescending & 0.938 & MTL \\
ucc & condescending & 0.938 & Vanilla \\
ucc & condescending & 0.940 & pretrained \\ 
 \hline
ucc & dismissive & 0.967 & CL \\
ucc & dismissive & 0.966 & MTL \\
ucc & dismissive & 0.966 & Vanilla \\
ucc & dismissive & 0.967 & pretrained \\ 
 \hline
ucc & generalisation & 0.981 & CL \\
ucc & generalisation & 0.981 & MTL \\
ucc & generalisation & 0.970 & Vanilla \\
ucc & generalisation & 0.981 & pretrained \\ 
 \hline
ucc & generalisation--unfair & 0.982 & CL \\
ucc & generalisation--unfair & 0.982 & MTL \\
ucc & generalisation--unfair & 0.981 & Vanilla \\
ucc & generalisation--unfair & 0.982 & pretrained \\ 
 \hline
ucc & healthy & 0.936 & CL \\
ucc & healthy & 0.926 & MTL \\
ucc & healthy & 0.921 & Vanilla \\
ucc & healthy & 0.936 & pretrained \\ 
 \hline
ucc & hostile & 0.978 & CL \\
ucc & hostile & 0.976 & MTL \\
ucc & hostile & 0.977 & Vanilla \\
ucc & hostile & 0.978 & pretrained \\ 
 \hline
ucc & sarcastic & 0.955 & CL \\
ucc & sarcastic & 0.955 & MTL \\
ucc & sarcastic & 0.955 & Vanilla \\
ucc & sarcastic & 0.954 & pretrained \\ 
 \hline
us--election & biden & 0.565 & CL \\
us--election & biden & 0.541 & MTL \\
us--election & biden & 0.501 & Vanilla \\
us--election & biden & 0.510 & pretrained \\ 
 \hline
us--election & hof & 0.897 & CL \\
us--election & hof & 0.907 & MTL \\
us--election & hof & 0.890 & Vanilla \\
us--election & hof & 0.897 & pretrained \\ 
 \hline
us--election & trump & 0.389 & CL \\
us--election & trump & 0.432 & MTL \\
us--election & trump & 0.375 & Vanilla \\
us--election & trump & 0.491 & pretrained \\ 
 \hline
\bottomrule
\end{tabular}


\begin{tabular}{llr}
\toprule
 & alg & nf1 \\
\midrule
0 & CL & 0.864495 \\
1 & MTL & 0.863886 \\
2 & Vanilla & 0.858456 \\
3 & pretrained & 0.875651 \\
\bottomrule
\end{tabular}

==> tables/old/proof_concept_final.tex <==
\begin{tabular}{rlll}
\toprule
em & task--name & task--detail & alg \\
\midrule
0.722656 & BAD4 & singlelabel & CL \\
0.736328 & BAD4 & singlelabel & MTL \\
0.726562 & BAD4 & singlelabel & Vanilla \\ 
 \hline
0.993194 & ghc & cv & CL \\
0.992514 & ghc & cv & MTL \\
0.960753 & ghc & cv & Vanilla \\ 
 \hline
0.920145 & ghc & hd & CL \\
0.890653 & ghc & hd & MTL \\
0.899501 & ghc & hd & Vanilla \\ 
 \hline
0.942604 & ghc & vo & CL \\
0.932396 & ghc & vo & MTL \\
0.914927 & ghc & vo & Vanilla \\ 
 \hline
0.929000 & multi & singlelabel & CL \\
0.912000 & multi & singlelabel & MTL \\
0.919333 & multi & singlelabel & Vanilla \\ 
 \hline
0.886485 & personal--attack & a & CL \\
0.932642 & personal--attack & a & MTL \\
0.868523 & personal--attack & a & Vanilla \\ 
 \hline
0.999957 & personal--attack & qa & CL \\
0.999957 & personal--attack & qa & MTL \\
0.999957 & personal--attack & qa & Vanilla \\ 
 \hline
0.928282 & personal--attack & ra & CL \\
0.952591 & personal--attack & ra & MTL \\
0.908981 & personal--attack & ra & Vanilla \\ 
 \hline
0.990371 & personal--attack & tpa & CL \\
0.985881 & personal--attack & tpa & MTL \\
0.981390 & personal--attack & tpa & Vanilla \\ 
 \hline
\bottomrule
\end{tabular}

\begin{tabular}{llr}
\toprule
 & alg & em \\
\midrule
0 & CL & 0.923633 \\
1 & MTL & 0.926107 \\
2 & Vanilla & 0.908881 \\
\bottomrule
\end{tabular}


==> tables/old/proof_of_concept_instant.tex <==
\begin{tabular}{rlll}
\toprule
em & task--name & task--detail & alg \\
\midrule
0.724609 & BAD4 & singlelabel & CL \\
0.789062 & BAD4 & singlelabel & Vanilla \\ 
 \hline
0.993421 & ghc & cv & CL \\
0.993421 & ghc & cv & CL \\
0.993421 & ghc & cv & CL \\
0.993421 & ghc & cv & CL \\
0.993421 & ghc & cv & Vanilla \\ 
 \hline
0.993421 & ghc & cv & Vanilla \\ 
 \hline
0.993421 & ghc & cv & Vanilla \\ 
 \hline
0.921279 & ghc & hd & CL \\
0.923775 & ghc & hd & Vanilla \\ 
 \hline
0.943058 & ghc & vo & CL \\
0.946688 & ghc & vo & Vanilla \\ 
 \hline
0.929000 & multi & singlelabel & CL \\
0.912000 & multi & singlelabel & MTL \\
0.924333 & multi & singlelabel & Vanilla \\ 
 \hline
0.941192 & personal--attack & a & CL \\
0.940674 & personal--attack & a & Vanilla \\ 
 \hline
0.999957 & personal--attack & qa & CL \\
0.999957 & personal--attack & qa & CL \\
0.999957 & personal--attack & qa & CL \\
0.999957 & personal--attack & qa & CL \\
0.999957 & personal--attack & qa & Vanilla \\ 
 \hline
0.999957 & personal--attack & qa & Vanilla \\ 
 \hline
0.999957 & personal--attack & qa & Vanilla \\ 
 \hline
0.999957 & personal--attack & qa & Vanilla \\ 
 \hline
0.955268 & personal--attack & ra & CL \\
0.960838 & personal--attack & ra & Vanilla \\ 
 \hline
0.990371 & personal--attack & tpa & CL \\
0.990371 & personal--attack & tpa & CL \\
0.990371 & personal--attack & tpa & CL \\
0.990803 & personal--attack & tpa & Vanilla \\ 
 \hline
0.990803 & personal--attack & tpa & Vanilla \\ 
 \hline
\bottomrule
\end{tabular}

==> tables/sensitivity-kshot.tex <==
\begin{tabular}{lllrl}
\toprule
task--name & task--detail & nf1 & k & alg \\
\midrule
cmsb & sexist & 0.793837 & 4 & CL \\
cmsb & sexist & 0.791636 & 8 & CL \\
cmsb & sexist & 0.735143 & 16 & CL \\
cmsb & sexist & 0.842993 & 32 & CL \\
cmsb & sexist & 0.856933 & 64 & CL \\ 
 \hline
ucc & antagonize & 0.762351 & 4 & CL \\
ucc & antagonize & 0.703750 & 8 & CL \\
ucc & antagonize & 0.848750 & 16 & CL \\
ucc & antagonize & 0.771250 & 32 & CL \\
ucc & antagonize & 0.802500 & 64 & CL \\ 
 \hline
ucc & condescending & 0.865000 & 4 & CL \\
ucc & condescending & 0.833125 & 8 & CL \\
ucc & condescending & 0.876250 & 16 & CL \\
ucc & condescending & 0.686250 & 32 & CL \\
ucc & condescending & 0.888750 & 64 & CL \\ 
 \hline
ucc & dismissive & 0.442500 & 4 & CL \\
ucc & dismissive & 0.663540 & 8 & CL \\
ucc & dismissive & 0.653750 & 16 & CL \\
ucc & dismissive & 0.607500 & 32 & CL \\
ucc & dismissive & 0.860000 & 64 & CL \\ 
 \hline
ucc & generalisation & 0.864375 & 4 & CL \\
ucc & generalisation & 0.786875 & 8 & CL \\
ucc & generalisation & 0.805000 & 16 & CL \\
ucc & generalisation & 0.713750 & 32 & CL \\
ucc & generalisation & 0.826250 & 64 & CL \\ 
 \hline
ucc & generalisation--unfair & 0.830000 & 4 & CL \\
ucc & generalisation--unfair & 0.795000 & 8 & CL \\
ucc & generalisation--unfair & 0.683750 & 16 & CL \\
ucc & generalisation--unfair & 0.801250 & 32 & CL \\
ucc & generalisation--unfair & 0.785625 & 64 & CL \\ 
 \hline
ucc & healthy & 0.575625 & 4 & CL \\
ucc & healthy & 0.706875 & 8 & CL \\
ucc & healthy & 0.628125 & 16 & CL \\
ucc & healthy & 0.520625 & 32 & CL \\
ucc & healthy & 0.746250 & 64 & CL \\ 
 \hline
ucc & hostile & 0.890000 & 4 & CL \\
ucc & hostile & 0.610000 & 8 & CL \\
ucc & hostile & 0.739375 & 16 & CL \\
ucc & hostile & 0.746250 & 32 & CL \\
ucc & hostile & 0.811875 & 64 & CL \\ 
 \hline
ucc & sarcastic & 0.614375 & 4 & CL \\
ucc & sarcastic & 0.827500 & 8 & CL \\
ucc & sarcastic & 0.611250 & 16 & CL \\
ucc & sarcastic & 0.756250 & 32 & CL \\
ucc & sarcastic & 0.765000 & 64 & CL \\ 
 \hline
us--election & hof & 0.676667 & 4 & CL \\
us--election & hof & 0.686667 & 8 & CL \\
us--election & hof & 0.656667 & 16 & CL \\
us--election & hof & 0.813333 & 32 & CL \\
us--election & hof & 0.886667 & 64 & CL \\ 
 \hline
\bottomrule
\end{tabular}

==> tables/tab_up_down.tex <==
\captionsetup[table]{skip=5pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[h]
\begin{tabular}{c|l}
\multirow{2}{*}{Upstream}       & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}CAD (4), Personal\_attack (4),  UCC (9),  GHC (3), \\  Multi, dygen-hate, abusive (2),  hate (2)\end{tabular}} \\
                                &                                                                                                                                                           \\
\multicolumn{1}{l|}{Downstream} &                                                                                                                                                          
\end{tabular}
\caption{Upstream and Downstream Tasks. }
\label{tab:up_down}
\end{table}

